Iterative Budgeted Exponential Search

We tackle two long-standing problems related to re-expansions in heuristic search algorithms. For graph search, A* can require $\Omega(2^{n})$ expansions, where $n$ is the number of states within the final $f$ bound. Existing algorithms that address this problem like B and B' improve this bound to $\Omega(n^2)$. For tree search, IDA* can also require $\Omega(n^2)$ expansions. We describe a new algorithmic framework that iteratively controls an expansion budget and solution cost limit, giving rise to new graph and tree search algorithms for which the number of expansions is $O(n \log C)$, where $C$ is the optimal solution cost. Our experiments show that the new algorithms are robust in scenarios where existing algorithms fail. In the case of tree search, our new algorithms have no overhead over IDA* in scenarios to which IDA* is well suited and can therefore be recommended as a general replacement for IDA*.

==> fig1.tex <==
\draw[dotted,opacity=0.5,thin] (7.500000,1.000000) -- (7.500000,-7.000000);
\draw[dotted,opacity=0.5,thin] (6.000000,1.000000) -- (6.000000,-7.000000);
\draw[dotted,opacity=0.5,thin] (5.500000,1.000000) -- (5.500000,-7.000000);
\draw[dotted,opacity=0.5,thin] (5.000000,1.000000) -- (5.000000,-7.000000);
\draw[dotted,opacity=0.5,thin] (4.500000,1.000000) -- (4.500000,-7.000000);
\draw[dotted,opacity=0.5,thin] (4.000000,1.000000) -- (4.000000,-7.000000);
\draw[dotted,opacity=0.5,thin] (3.500000,1.000000) -- (3.500000,-7.000000);
\draw[dotted,opacity=0.5,thin] (2.700000,1.000000) -- (2.700000,-7.000000);
\draw[dotted,opacity=0.5,thin] (2.600000,1.000000) -- (2.600000,-7.000000);
\draw[dotted,opacity=0.5,thin] (2.500000,1.000000) -- (2.500000,-7.000000);
\draw[dotted,opacity=0.5,thin] (1.800000,1.000000) -- (1.800000,-7.000000);
\draw[dotted,opacity=0.5,thin] (1.300000,1.000000) -- (1.300000,-7.000000);
\draw[dotted,opacity=0.5,thin] (0.800000,1.000000) -- (0.800000,-7.000000);
\draw[dotted,opacity=0.5,thin] (0.600000,1.000000) -- (0.600000,-7.000000);
\draw[dotted,opacity=0.5,thin] (0.500000,1.000000) -- (0.500000,-7.000000);
\draw[draw=none,fill=black,opacity=0.2] (4.500000,1.000000) rectangle (5.000000,-7.000000);
\draw[] (0.200000, 0.100000) -- (0.200000, 0.900000);
\draw[-latex] (0.200000, 0.500000) -- (10, 0.500000);
\node[ya] at (0.200000,0.500000) { $\cost_{\low}$ };
\draw[thick,red] (0.400000,0.333333) -- (0.400000,0.666667);\node[ya,circle,fill=blue!30!white,opacity=0.5] at (-1,0.500000) { 0 };
\draw[] (0.400000, -0.900000) -- (0.400000, -0.100000);
\draw[-latex] (0.400000, -0.500000) -- (10, -0.500000);
\node[ya] at (0.400000,-0.500000) { $\cost_{\low}$ };
\draw[thick,red] (0.800000,-0.666667) -- (0.800000,-0.333333);\node[ya,circle,fill=blue!30!white,opacity=0.5] at (-1,-0.500000) { 1 };
\draw[] (0.800000, -1.900000) -- (0.800000, -1.100000);
\draw[-latex] (0.800000, -1.500000) -- (10, -1.500000);
\node[ya] at (0.800000,-1.500000) { $\cost_{\low}$ };
\draw[thick,red] (1.600000,-1.666667) -- (1.600000,-1.333333);\node[ya,circle,fill=blue!30!white,opacity=0.5] at (-1,-1.500000) { 2 };
\draw[] (1.600000, -2.900000) -- (1.600000, -2.100000);
\draw[-latex] (1.600000, -2.500000) -- (10, -2.500000);
\node[ya] at (1.600000,-2.500000) { $\cost_{\low}$ };
\draw[thick,red] (3.200000,-2.666667) -- (3.200000,-2.333333);\node[ya,circle,fill=blue!30!white,opacity=0.5] at (-1,-2.500000) { 3 };
\draw[] (3.200000, -3.900000) -- (3.200000, -3.100000);
\draw[-latex] (3.200000, -3.500000) -- (10, -3.500000);
\node[ya] at (3.200000,-3.500000) { $\cost_{\low}$ };
\draw[thick,red] (6.400000,-3.666667) -- (6.400000,-3.333333);\node[ya,circle,fill=red!30!white,opacity=0.5] at (-1,-3.500000) { 4 };
\draw[thick,red] (4.600000,-4.666667) -- (4.600000,-4.333333);\draw[] (3.200000, -4.900000) -- (3.200000, -4.100000);
\draw[] (6.000000, -4.900000) -- (6.000000, -4.100000);
\draw[] (3.200000, -4.500000) -- (6.000000, -4.500000);
\node[ya] at (3.200000,-4.500000) {$\cost_{\low}$};
\node[anchor=west,font=\scriptsize] at (6.000000,-4.500000) {$\cost_{\high}$};
\node[ya,fill=blue!30!white,opacity=0.5,circle] at (-1,-4.500000) { 5 };
\draw[thick,red] (5.300000,-5.666667) -- (5.300000,-5.333333);\draw[] (4.600000, -5.900000) -- (4.600000, -5.100000);
\draw[] (6.000000, -5.900000) -- (6.000000, -5.100000);
\draw[] (4.600000, -5.500000) -- (6.000000, -5.500000);
\node[ya] at (4.600000,-5.500000) {$\cost_{\low}$};
\node[anchor=west,font=\scriptsize] at (6.000000,-5.500000) {$\cost_{\high}$};
\node[ya,fill=red!30!white,opacity=0.5,circle] at (-1,-5.500000) { 6 };
\draw[thick,red] (4.800000,-6.666667) -- (4.800000,-6.333333);\draw[] (4.600000, -6.900000) -- (4.600000, -6.100000);
\draw[] (5.000000, -6.900000) -- (5.000000, -6.100000);
\draw[] (4.600000, -6.500000) -- (5.000000, -6.500000);
\node[ya] at (4.600000,-6.500000) {$\cost_{\low}$};
\node[anchor=west,font=\scriptsize] at (5.000000,-6.500000) {$\cost_{\high}$};
\node[ya,fill=blue!30!white,opacity=0.5,circle] at (-1,-6.500000) { 7 };
\node[anchor=north] at (4.750000,2.5) {critical region};
\draw[-latex] (4.750000,1.5) -- (4.750000,1);
\node[anchor=north] at (0.400000,2.5) {query};
\draw[-latex] (0.400000,1.5) -- (0.400000,1);


==> fig2.tex <==
\draw[draw=none,fill=black,opacity=0.2] (12.000000, 0.000000) rectangle (15.000000, -12.000000);
\draw[] (20.000000, 0.000000) -- (20.000000, -0.200000);
\draw[] (19.000000, 0.000000) -- (19.000000, -0.200000);
\draw[] (18.000000, 0.000000) -- (18.000000, -0.200000);
\draw[] (17.000000, 0.000000) -- (17.000000, -0.200000);
\draw[] (16.000000, 0.000000) -- (16.000000, -0.200000);
\draw[] (15.000000, 0.000000) -- (15.000000, -0.200000);
\draw[] (14.000000, 0.000000) -- (14.000000, -0.200000);
\draw[] (13.000000, 0.000000) -- (13.000000, -0.200000);
\draw[] (12.000000, 0.000000) -- (12.000000, -0.200000);
\draw[] (11.000000, 0.000000) -- (11.000000, -0.200000);
\draw[] (10.000000, 0.000000) -- (10.000000, -0.200000);
\draw[] (9.000000, 0.000000) -- (9.000000, -0.200000);
\draw[] (8.000000, 0.000000) -- (8.000000, -0.200000);
\draw[] (7.000000, 0.000000) -- (7.000000, -0.200000);
\draw[] (6.000000, 0.000000) -- (6.000000, -0.200000);
\draw[] (5.000000, 0.000000) -- (5.000000, -0.200000);
\draw[] (4.000000, 0.000000) -- (4.000000, -0.200000);
\draw[] (3.000000, 0.000000) -- (3.000000, -0.200000);
\draw[] (2.000000, 0.000000) -- (2.000000, -0.200000);
\draw[] (1.000000, 0.000000) -- (1.000000, -0.200000);
\draw[] (0.000000, 0.000000) -- (0.000000, -12.000000);
\node[anchor=east,fill=white] at (3.000000, -1.000000) { $\cost_{\texttt{low}}$ };
\draw[] (3.000000, -0.333333) -- (3.000000, -1.666667);
\draw[-latex] (3.000000, -1.000000) -- (21.000000, -1.000000);
\node[circle,draw] at (-1.500000, -1.000000) { 1 };
\draw[fill=black,draw=none] (4.000000, -1.000000) circle (0.160000);
\node[anchor=east,fill=white] at (5.000000, -3.000000) { $\cost_{\texttt{low}}$ };
\draw[] (5.000000, -2.333333) -- (5.000000, -3.666667);
\draw[-latex] (5.000000, -3.000000) -- (21.000000, -3.000000);
\node[circle,draw] at (-1.500000, -3.000000) { 2 };
\draw[fill=black,draw=none] (5.000000, -3.000000) circle (0.160000);
\node[anchor=east,fill=white] at (6.000000, -5.000000) { $\cost_{\texttt{low}}$ };
\draw[] (6.000000, -4.333333) -- (6.000000, -5.666667);
\draw[-latex] (6.000000, -5.000000) -- (21.000000, -5.000000);
\node[circle,draw] at (-1.500000, -5.000000) { 3 };
\draw[fill=black,draw=none] (7.000000, -5.000000) circle (0.160000);
\node[anchor=east,fill=white] at (8.000000, -7.000000) { $\cost_{\texttt{low}}$ };
\draw[] (8.000000, -6.333333) -- (8.000000, -7.666667);
\draw[-latex] (8.000000, -7.000000) -- (21.000000, -7.000000);
\node[circle,draw] at (-1.500000, -7.000000) { 4 };
\draw[fill=black,draw=none] (11.000000, -7.000000) circle (0.160000);
\node[anchor=east,fill=white] at (12.000000, -9.000000) { $\cost_{\texttt{low}}$ };
\draw[] (12.000000, -8.333333) -- (12.000000, -9.666667);
\draw[-latex] (12.000000, -9.000000) -- (21.000000, -9.000000);
\node[circle,draw,fill=black!20!white] at (-1.500000, -9.000000) { 5 };
\draw[fill=black,draw=none] (19.000000, -9.000000) circle (0.160000);
\node[anchor=east,fill=white] at (12.000000, -11.000000) { $\cost_{\texttt{low}}$ };
\draw[] (12.000000, -10.333333) -- (12.000000, -11.666667);
\node[anchor=west] at (19.000000, -11.000000) { $\cost_{\texttt{high}}$ };
\draw[] (19.000000, -10.333333) -- (19.000000, -11.666667);
\draw[] (12.000000, -11.000000) -- (19.000000, -11.000000);
\node[circle,draw] at (-1.500000, -11.000000) { 6 };
\draw[fill=black,draw=none] (15.000000, -11.000000) circle (0.160000);
\node[anchor=south] at (0.000000, 0.100000) { $0$ };
\draw[-latex] (0.000000, 0.000000) -- (21.000000, 0.000000);
\node[anchor=west] at (21.000000, 0.000000) { $\cost$ };

